Sensitivity analysis of fractional linear systems based on random walks with negligible memory usage

A random walk-based method is proposed to efficiently compute the solution of a large class of fractional in time linear systems of differential equations (linear F-ODE systems), along with the derivatives with respect to the system parameters. Such a method is unbiased and unconditionally stable, and can therefore be used to provide an unbiased estimation of individual entries of the solution, or the full solution. By using stochastic differentiation techniques, it can be used as well to provide unbiased estimators of the sensitivities of the solution with respect to the problem parameters without any additional computational cost. The time complexity of the algorithm is discussed here, along with suitable variance bounds, which prove in practice the convergence of the algorithm. Finally, several test cases were run to assess the validity of the algorithm.

==> apendices.tex <==
\begin{appendices}
\section{The pathspace}
\label{appendix:B}
We consider as the hidden probability space $(\Omega,\mathcal{F},\mathbb{P})$ the idealized RNG stream of the computer $\Omega =\otimes^\infty_{i=1} [0,1]$ the sigma-algebra generated by the subsets $\otimes_{i=1}^n[a_i,b_i]$ and the completion of the measure $\mathbb{P}(\otimes[a_i,b_i]_{i=1}^n)=\prod_{i=1}^n (b_i - a_i)$. Then, we consider the path function that takes the RNG stream to a random walk
\begin{equation}
    {\rm{path}}_{\theta}(\omega)=\{(S_i(u_{2i+1};\theta),\Delta \tau_i(u_{2i+3};\theta) )\}_{i=1}^\infty\in  \times \prod_{i=1}^\infty(\bm{S}\times \mathbb{R}_+)
\end{equation}
where the random walk is completely determined by the states $S_i\in\bm{S}$ and the sojourn times $\Delta \tau_i>0$. Writing $S_i({\rm{path}}_{\theta}(\omega))$ and $\Delta \tau_i({\rm{path}}_{\theta}(\omega))$ refers just to the $i$-th state and $i$-th sojourn time of the random walk respectively, and for clarity we just write $S_i$ and $\Delta \tau_i$. 

To match the Malliavin weight notation, we take the stochastic process viewpoint. We define the path process $\Gamma_t\colon [0,\infty)\rightarrow\bm{S}=\{1,\dots, n\}$ as 
\begin{equation}
    \Gamma_{\theta}(\omega,t)=S_{1+\nu_{\theta}(\omega,t)}({\rm{path}}_{\theta}(\omega))
\end{equation}
Where the dual process $\nu_t$ is given by
\begin{equation}
    \nu_{\theta}(\omega,t)=\max_i\left[ \sum_{k=1}^i {\Delta \tau_k}({\rm{path}}_{\theta}(\omega))<t\right]
\end{equation}
The solution to a F-ODE $u_i(T;\theta)$ is then, formally, the expected value of some functional $J_T({\rm{path}}_{\theta}(\omega);\theta)$
\begin{align}
\label{expected-value}
    &u_i(T)=\mathbb{E}(J_T({\rm{path}}_{\theta}(\omega);\theta)\vert S_1({\rm{path}}_{\theta}(\omega))=i)\nonumber\\
\end{align}
where the functional is given by
\begin{align*}
\label{eq:functional}
    J_T({\rm{path}}_{\theta}(\omega);\theta)&=u_{\Gamma(\omega,T)}(0)\prod_{i=1}^{\nu(\omega,T)}\frac{\mathrm{sgn}(A_{S_i,S_{i+1}})\sum_{j\neq S_i}\mathrm{sgn}(A_{S_{i}j})A_{S_{i}j}}{-A_{S_i,S_i}}\nonumber\\
    &=u_{\Gamma(\omega,T)}(0)\prod_{i=1}^{\nu(\omega,T)}\chi(S_i,S_{i+1})
\end{align*}
We drop dependence on $\omega$ and $\theta$ whenever its clear enough.

To perform Malliavin weights, we need some kind of density function for the pathspace. In order to achieve that, we quotient the measure space $\Omega_T=\Omega/{\sim}$ where two random walks ${\rm{path}}_{\theta}(\mathbf{u_1})$ and ${\rm{path}}_{\theta}(\mathbf{u_2})$ are equivalent if they are equal in $[0,T]$. In this formulation paths are completely determined by
\begin{equation}
    {\rm{path}}_{\theta}(\omega)=\{S_i,\Delta \tau_i\}_{i=1}^{1+\nu(T)}
\end{equation}
and we can take expected values of functionals by integrating over the complete RNG stream
\begin{equation}
    \mathbb{E}(J({\rm{path}}_{\theta}(\omega)))=\int_{\otimes^\infty_{i=1} [0,1]} d\omega\; J({\rm{path}}(\omega);{\theta})p_{\theta}({\rm{path}}(\omega))
\end{equation}
where now dependency of parameters is shifted to the probability density given by the Radon-Nykodym theorem
\begin{equation}
    p({\rm{path}}_{\theta}(\omega))=\mathbb{P}(\xi(S_{1+\nu(T)})>\Delta \tau_{1+\nu(T)})\prod_{i=1}^{\nu_T}\mathbb{P}(\xi(S_i)=\Delta \tau_i)\mathbb{P}(J_{S_i}=S_{i+1})
\end{equation}
where sojourn times at state $i$ are $\xi(S_i)$-distributed, and $J_{S_i}$ is a random variable taking values in $\{1,\dots,n\}/i$, which is the probability of jumping to a new state $i+1$.
%%=============================================%%
%% For submissions to Nature Portfolio Journals %%
%% please use the heading ``Extended Data''.   %%
%%=============================================%%

%%=============================================================%%
%% Sample for another appendix section			       %%
%%=============================================================%%

%% \section{Example of another appendix section}\label{secA2}%
%% Appendices may be used for helpful, supporting or essential material that would otherwise 
%% clutter, break up or be distracting to the text. Appendices can consist of sections, figures, 
%% tables and equations etc.

\end{appendices}

==> trash/adjoint.tex <==
\section{Derivation of the adjoint method}\label{appendix:B}
For a modern introduction of sensitivity analysis from a deterministic point of view we refer to \cite{kaltenbacher2023inverse}. Suppose we have a continuous set of observations 
\begin{equation}
    \mathbf{u}(\,\cdot\,;\text{obs})\colon [0,T] \longrightarrow\mathbb{R}^N
\end{equation}
over the whole grid (the adjoint method for partial observations in $\mathbb{R}^S\subset\mathbb{R}^N$ also admits the following solution but full solution still needs to be computed). We consider the problem
\begin{align}
\min_{\bm{\alpha} \in [0,1]^n} \mathcal{L}(\bm{\alpha}) &= \int_0^T dt\;\frac{1}{2}\| \mathbf{u}(t;\bm{\alpha}) - \mathbf{u}(t;\text{obs}) \|^2 \nonumber \\
\text{subject to}\quad & ^C_0 D_t^{\bm{\alpha}}\mathbf{u}(t;\mathbf{\alpha}) = \mathbf{A}\mathbf{u}(t;\alpha),\quad \mathbf{u}(0;\bm{\alpha})=\mathbf{u}(0;\text{obs})
\label{adjoint-constraint}
\end{align}
The adjoint method consists in loading the constraint onto the loss with the help of an auxiliary function $\bm{\lambda}(\cdot)\colon[0,T]\longrightarrow \mathbb{R}^N$
\begin{equation}
    \mathcal{L}(\bm{\alpha}) = \int_0^T dt\;\left[ \frac{1}{2}\Vert \mathbf{u}(t;\bm{\alpha})-\mathbf{u}(t;\text{obs})\Vert^2+\bm{\lambda}(t)^T\left(^C_0 D_t^{\bm{\alpha}}\mathbf{u}(t;\mathbf{\alpha}) - \mathbf{A}\mathbf{u}(t;\alpha) \right)\right]
\end{equation}
while maintaining the constraint in \ref{adjoint-constraint}. For clarity purposes, we drop dependency on vector $\bm{\alpha}$. Taking the derivative of the loss
\begin{equation}
    \frac{d\mathcal{L}}{d\bm{\alpha}}=\int_0^T dt\; \left[( \mathbf{u}(t)-\mathbf{u}(t;\text{obs}))\frac{d\mathbf{u}(t)}{d\bm{\alpha}}+\bm{\lambda}(t)^T\left(\frac{d(^C_0 D_t^{\bm{\alpha}}\mathbf{u}(t;\mathbf{\alpha}))}{d\bm{\alpha}}-\mathbf{A} \frac{d\mathbf{u}(t)}{d\bm{\alpha}} \right)\right]
    \label{adjoint-a4}
\end{equation}
In the classical adjoint method for an ODE constraint, one would use the integration by parts formula to get rid of the derivative in time
\begin{equation}
    \int_0^T dt\; \bm{\lambda}(t)^T\frac{d}{dt}\frac{d\mathbf{u}}{d\bm{\theta}}=\bm{\lambda}(T)^T\mathbf{u}(T)-\bm{\lambda}(0)^T\mathbf{u}(0)-\int_0^T dt\;\frac{d\bm{\lambda}^T}{dt}\frac{d\mathbf{u}}{d\bm{\theta}}
\end{equation}
In a similar way, for a F-ODE constraint, we want to make use of the fractional integration by parts formula \cite{hendy2022cole} which in the scalar case is given by
\begin{equation}
    \int_0^T f(t) ^C_0 D_t^\alpha g(t) = \left[ g(t) \; _t I_T^{1-\alpha}f(t)\right]_0^T+\int_0^T g(t) \; _t^{RL} D_T^\alpha f(t) dt
\end{equation}
However, as the order of the fractional derivative is the parameter itself, we cannot apply the chain rule right away. Using the following scalar identity
\begin{equation}
    \frac{d}{d\alpha}\frac{t^{-\alpha}}{\Gamma(1-\alpha)}=\frac{t^{-\alpha}(\psi^{(0)}(1-\alpha)-\log(t))}{\Gamma{(1-\alpha})}
\end{equation}
where $\psi^{(0)}(\alpha)=\frac{d}{d\alpha}\log(\Gamma(\alpha))$ is the digamma function, we can expand the sensitivity of the Caputo fractional derivative as
\begin{align}
\frac{d(^C_0 D_t^{\bm{\alpha}} u)}{d\bm{\alpha}}= &
\frac{d}{d\bm{\alpha}}\int_{0}^t d\tau \frac{(t-\tau)^{-\bm{\alpha}}}{\Gamma(1-\bm{\alpha})} \frac{\partial \mathbf{u}(t;\bm{\alpha})}{\partial t}(\tau) \nonumber \\
&=\;^C_0 D_t^{\bm{\alpha}} \frac{d\mathbf{u}}{d\bm{\alpha}}+\int_0^t d\tau\; \frac{(t-\tau)^{-\bm{\alpha}}(\psi^{(0)}(1-\bm{\alpha})-\log(t-\tau))}{\Gamma{(1-\bm{\alpha}})}\frac{\partial \mathbf{u}}{\partial s}(\tau) \nonumber \\
&=\;^C_0 D_t^{\bm{\alpha}} \frac{d\mathbf{u}}{d\bm{\alpha}}+\psi^{(0)}(1-\bm{\alpha}) ^C_0 D_t^{\bm{\alpha}} \mathbf{u} -\int_0^t d\tau\; \frac{(t-\tau)^{-\bm{\alpha}}\log(t-\tau)}{\Gamma(1-\bm{\alpha})}\frac{\partial \mathbf{u}}{\partial s}(\tau)\nonumber \\
&=\;^C_0 D_t^{\bm{\alpha}} \frac{d\mathbf{u}}{d\bm{\alpha}}+\psi^{(0)}(1-\bm{\alpha}) \mathbf{A} \mathbf{u} -\int_0^t d\tau\; \frac{(t-\tau)^{-\bm{\alpha}}\log(t-\tau)}{\Gamma(1-\bm{\alpha})}\frac{\partial \mathbf{u}}{\partial s}(\tau)\nonumber\\
&=\;^C_0 D_t^{\bm{\alpha}} \frac{d\mathbf{u}}{d\bm{\alpha}}+\Gamma(\mathbf{u},t;\bm{\alpha})
\label{dcaputodalpha}
\end{align}
where we assume that the following derivatives can be interchanged
$$\frac{d}{d\bm{\alpha}}\frac{\partial \mathbf{u}}{\partial s}=\frac{\partial}{\partial s}\frac{d\mathbf{u}}{d\bm{\alpha}}
$$
that constraint \ref{adjoint-constraint} holds, the notation $^C_0 D_t^{\bm{\alpha}} \frac{d\mathbf{u}}{d\bm{\alpha}}$ should be understood as the Caputo derivative of order $\alpha_i$ acting over the $i$-th row of the sensitivity matrix. Notice how the quantities that are known by solving the original F-ODE \ref{adjoint-constraint} are written by a $\Gamma$. Finally, equation

\begin{equation}
    \frac{d\mathcal{L}}{d\bm{\alpha}}=\int_0^T dt\; \left[( \mathbf{u}(t)-\mathbf{u}(t;\text{obs}))^T\frac{d\mathbf{u}(t)}{d\bm{\alpha}}+\bm{\lambda}(t)^T\left(^C_0 D_t^{\bm{\alpha}}\frac{d\mathbf{u}(t)}{d\bm{\alpha}}+\Gamma(\mathbf{u},t;\bm{\alpha})-\mathbf{A} \frac{d\mathbf{u}(t)}{d\bm{\alpha}} \right)\right]
    \label{adjoint-subs}
\end{equation}
and using integration by parts entry by entry in the following vector-valued equation
$$
\int_0^T \lambda_i(t) \; ^C_0 D_t^{\alpha_i} \frac{d\mathbf{u}(t)}{d\alpha_j} = \left[ \frac{d\mathbf{u}(t)}{d\alpha_j} \; _t I_T^{1-{\alpha_i}}\lambda_i(t)\right]_0^T+\int_0^T \frac{d\mathbf{u}(t)}{d\alpha_j} \; _t^{RL} D_T^{\alpha_i} \lambda_i(t) dt
$$
By noting that $\frac{d\mathbf{u}(0;\alpha)}{d\alpha_j}=0$ and requiring that $ _T I_T^{1-{\alpha_i}}\lambda_i(T)=0$---which in this case is equivalent to $\bm{\lambda}(T)=0$, but not in general, see \cite{hendy2022cole}---the loss becomes
\begin{align}
    \frac{d\mathcal{L}}{d\bm{\alpha}}&=\int_0^T dt\; \left[( \mathbf{u}(t)-\mathbf{u}(t;\text{obs})-\mathbf{A}\bm{\lambda}(t))^T\frac{d\mathbf{u}(t)}{d\alpha}+\sum_{i=1}^N  \frac{du_i(t)}{d\bm{\alpha}} \; _t^{RL} D_T^{\alpha_i} \lambda_i(t) +\bm{\lambda}(t)^T\Gamma(\mathbf{u},t,\bm{\alpha}) \right]
\end{align}
If we force the auxiliary function $\bm{\lambda}(t)$ to solve the backwards equation
$$
_t^{RL} D_T^{\alpha_i} \bm{\lambda}(t)=\mathbf{A}^T \bm{\lambda}(t)-( \mathbf{u}(t;\alpha)-\mathbf{u}(t;\text{obs})),\quad \bm{\lambda}(T)=0
$$
by numerically solving for $\mathbf{u}(t;\bm{\alpha})$ and $\bm{\lambda}(t)$, we can evaluate the sensitivities as 
\begin{align*}
    \frac{d\mathcal{L}}{d\bm{\alpha}}&=\int_0^T dt\; \bm{\lambda}(t)^T \Gamma(\mathbf{u},t,\bm{\alpha})
\end{align*}

==> trash/variance_explosion.tex <==
\subsubsection{Variance explosion and reverting dynamics}
This then leads to the issue of dealing with a FPDE of the form
\begin{align}
    &^C_0 D^{\alpha(x)}_t u(x,t) = \mathscr{L} u(x,t)\quad (x,t)\in\Omega\times[0,T]\nonumber\\
    &u(x,0)=\exp(-(x-\mu)^2/2\sigma^2)
\end{align}
when dealing with Gaussian pulses in inverse problems, as in optical tomography: the narrower the Gaussian pulse and the more finer the mesh we take for $\Omega$, the worse the worst-case scenario bound we gave.
Further work should go here but we believe the correct way to deal with this is to find a representation that throws trajectories from the node corresponding to $\mu$ for delta-like initial conditions $u(x,0)=\delta(x-\mu)$, this is known to be doable by taking the transpose of the infinitesimal generator $\mathbf{Q}^T$ in continuous time Markov-chains to create dynamics in reversed time, but we have not explored yet how to deal with Semi-Markov processes and their sensitivities, as non-Markovianity in time needs some careful treatment \cite{ertel2022operationally}. Furthermore, we do not believe this time reveresion to be possible with signed matrices, we believe $\mathbf{A}$ should be adequately discretizing an elliptic operator so that we can give an Ito diffusion meaning.
